Machine Learning-based Test Selection for Simulation-based Testing of Self-driving Cars Software

Simulation platforms facilitate the development of emerging Cyber-Physical Systems (CPS) like self-driving cars (SDC) because they are more efficient and less dangerous than field operational test cases. Despite this, thoroughly testing SDCs in simulated environments remains challenging because SDCs must be tested in a sheer amount of long-running test cases. Past results on software testing optimization have shown that not all the test cases contribute equally to establishing confidence in test subjects' quality and reliability, and the execution of "safe and uninformative" test cases can be skipped to reduce testing effort. However, this problem is only partially addressed in the context of SDC simulation platforms. In this paper, we investigate test selection strategies to increase the cost-effectiveness of simulation-based testing in the context of SDCs. We propose an approach called SDC-Scissor (SDC coSt-effeCtIve teSt SelectOR) that leverages Machine Learning (ML) strategies to identify and skip test cases that are unlikely to detect faults in SDCs before executing them. Our evaluation shows that SDC-Scissor outperforms the baselines. With the Logistic model, we achieve an accuracy of 70%, a precision of 65%, and a recall of 80% in selecting tests leading to a fault and improved testing cost-effectiveness. Specifically, SDC-Scissor avoided the execution of 50% of unnecessary tests as well as outperformed two baseline strategies. Complementary to existing work, we also integrated SDC-Scissor into the context of an industrial organization in the automotive domain to demonstrate how it can be used in industrial settings.

==> BeamNG-background.tex <==
\BNG is a framework specializing in autonomous driving and driver's training. It has been recently released under a mix of commercial and open-source licenses by \BNGC.\footnote{\BNG is available at \url{https://beamng.gmbh/research/} and is free for non-commercial use.}
%
The framework features a powerful soft-body simulator, several editors (e.g., road editors, track generator, world editor), and an extensive API that enables procedural content generation, automatic collection of simulation data for training and validation, and control of simulated vehicles using external programs (e.g., driving AIs).
%
%Additionally, since \BNG is derived from a video-game developed by the same company, the framework \begin{inparaenum}[(i)]
%\item comes with an unmatched set of assets, including more than twenty vehicles, seven trailers, hundreds of obstacles, elements of scenery and types of vegetation, and seventeen detailed maps scoring forty-four square kilometers of urban and suburban environments;
% 11 brands, 25 models (1 to be released)
% trailers:
% 2 brands, 7 models
% levels: 17 maps with more than 27136 km^2
%\item it is well maintained and meets stringent requirements on real-time execution and visual realism;
%\item the majority of its components are open-source\footnote{The Lua code is open-source under the CDDL or MIT licenses but the C++ core simulator is not.} and extensible;
%and, \item it has a large user base that continuously provides fresh and diverse content, extensions, \emph{mods}, and add-ons.
%\end{inparaenum} 

In this section, we briefly describe \BNG's software architecture and main components, its approach to soft-body simulation (Section~\ref{sec:beamng-simulation}), and how part of its APIs (i.e., \BNGPY) can be used to procedurally generate environments and test scenarios (Section~\ref{sec:beamngpy}).

\subsection{\BNG's Architecture}
\label{sec:swarchitecture}

\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{beamng_architecture.eps}
    \vspace{-2mm}
    \caption{Overview of \BNG}
    \label{fig:swarchitecture}
    \vspace{-3mm}
\end{figure}
%
\BNG is organized around a central \emph{game engine} that communicates with the \emph{physics simulation}, the \emph{UI}, and the \emph{\BNGPY API}\footnote{\BNGPY is available as a package from PyPI, the Python Package Index, while its source code is available at \url{https://github.com/BeamNG/BeamNGpy}} as exemplified by Figure~\ref{fig:swarchitecture}.
%
CPS' developers and testers can use \BNG via its UI or API.
%
The UI can be used for game control, and its diverse editors enable assets and content creation (e.g., \emph{gameplay}, \emph{scenarios}).
For example, developers can use the world editor to create or modify the virtual environments that are used in the simulations, while testers can create 
test scripts (\emph{gameplay} in the figure) to setup dynamic scenarios.
%
The API, instead, allows the automated generation and execution of test scenarios, the collection of simulation data for training as well as testing and validating CPSs (e.g., camera images, LIDAR point clouds, g-forces), and the possibility to interact with the running simulation (e.g., drive vehicles, move objects around).
%
The \emph{game engine} manages the simulation setup, camera, graphics, sounds, gameplay, and overall resource management. The \emph{physics core} handles resource-intensive tasks such as collision detection, basic physics simulation and orchestrates the multi-threaded execution of the vehicle simulators (see Section~\ref{sec:beamng-simulation}). The \emph{vehicle simulators} ---one for each of the simulated vehicles--- simulate the high-level driving functions and the various vehicle sub-systems (e.g., drivetrain, ABS, ESC, Turbo).

%\subsection{\BNG's Code Base}
%\BNG is implemented using various technologies but primarily consists of C++ and Lua code.
%The framework code base contains more than 350k lines of C++ code and more than 200K lines of Lua code (without considering third-party libraries). The physics simulation alone accounts for some 10k lines of C++ code.

\subsection{\BNG's Soft-body Simulation}
\label{sec:beamng-simulation}
This section describes how \BNG implements the physics simulation.

\textbf{The Core Physics Model}.
At its very core, \BNG implements the fundamental spring-mass model. 
% ALESSIO: This is confusing: are there other "simulators"? are they soft-body? what physics phenomena do they simulate? 
%Surrounding this core model are a variety of simulators that target other physics phenomena.
%
In its basic form, this model consists of \emph{nodes} with mass connected by weightless elastic elements, called \textit{beams}.
Beams implement a parallel mass-spring-damper circuit and obey Hooke's law extended with damping:
%
\begin{equation}
    F_{s} = -kx - c\dot{x} \label{eq:hooke-law}
\end{equation}
%
According to this law, the force $F_{s}$ necessary to extend or compress a spring by some distance $x$ is proportional to that distance by a positive factor $k$ that characterizes the spring's stiffness. Damping, instead, is a force that opposes the spring's motion and is proportional to the spring' velocity $(\dot{x})$ by a positive factor $c$ that characterizes the spring's internal friction.
%
Therefore, the mass-spring model can simulate how forces applied to the nodes propagate through the beams causing them to expand, compress, deform, or even break.

\begin{figure}[tp]
    \centering
    \includegraphics[width=0.40\columnwidth]{car-beams.png}
    \hspace{1.5cm}
    \includegraphics[width=0.40\columnwidth]{car-triangles}
    \caption{An example of how \BNG models the internal (left panel) and the external (right panel) structure of vehicles. The internal structure is modeled as a three-dimensional network of nodes and beams, while the external structure consists of triangles.}
    \label{fig:car-beams}
    \vspace{-3mm}
\end{figure}

\emph{Nodes} are dimensionless mass-points that occupy a position in space and are affected by the sum of forces propagated by the elastic elements that connect them. Since \BNG does not model nodes' rotation, nodes do not sum any momentum; hence, they act as hinges free in all axes. 
Nevertheless, nodes have frictional properties and collide against other simulated entities.
%
Nodes can be organized along one dimension to form chains, two dimensions to form polygonal meshes modeling the edges of objects' surfaces, or three dimensions to form complex networks modeling the internal structure of bodies~\cite{Dalboni}.
%
Figure~\ref{fig:car-beams} (left panel) exemplifies how the body of a vehicle is modeled as a three-dimensional network in \BNG.

\emph{Beams and triangles} connect nodes. Beams enable the simulation of bodies' deformation, while triangles enable the simulation of aerodynamic' drag, lift and the simulation of enclosed pressured surfaces. 
Additionally, triangles enable detecting collisions and computing collision response.
%
Figure~\ref{fig:car-beams} (right panel) highlights how the triangles contribute to the vehicle's body modeling in \BNG.
%
To help developers build accurate models that involve linear and non-linear behaviors typical of real-life components, \BNG defines various types of beams. Noticeably, this is one of the most distinctive novelties of the framework. 
%
\emph{Basic beams} have constant spring and damping rates, hence implement the linear behavior of Hooke's law (see Equation~\ref{eq:hooke-law}).
They can stretch, shrink, break, or permanently deform and can be used to model various materials by adjusting their deformation and break thresholds.
%
\emph{Bounded beams}, instead, have different spring and damp rates depending on how fast ---not how much--- they are compressed or expanded. They simulate materials with non-linear properties, like real-life car suspension's spring and dampers, and might have a defined length to limit suspension's travel.
%
\emph{Anisotropic beams} implement different behaviors during compression and expansion~\cite{anisotropic:beams}. They can be used to model structures that are easy to compress but very hard to expand, such as a tire's sidewall, and ``supporting'' structures that resist compression but are free to expand.
%
Finally, \emph{L-beams} and \emph{torsion bars} model angular springs and can be used to simulate the leaf springs in real-life suspension systems.

\begin{figure}[tp]
    \centering
    \includegraphics[width=0.40\columnwidth]{car-exploded.jpg}
    \includegraphics[width=0.40\columnwidth]{suspensions-beams.png}
    \caption{An example of a \BNG's vehicle model. The vehicle is composed of different parts that are assembled to resemble real-life settings. The 3d graphic meshes of these parts are presented in (left panel). The vehicle physics design contains 714 nodes that are connected by 4479 beams of various types and 976 triangles. The rear suspension part is presented in (right panel).}
    \label{fig:car-exploded}
    \vspace{-3mm}
\end{figure}
%
\textbf{The Vehicle Models.}
The diversified types of \BNG's beams allow developers to accurately model complex systems, such as complete vehicles. 
%
To facilitate reusability and maintainability, \BNG models vehicles as ensembles of individual components that correspond to real-life vehicle's part (see Figure~\ref{fig:car-exploded}).
%
Not all the components are modeled at the same level of detail. Some components, such as wheels and suspensions, are modeled as beams and nodes to accurately simulate their physics. Other components, instead, are modeled only in abstract form; for instance, this is the case of vehicles' engine.
%
Figure~\ref{fig:car-exploded} illustrates the main components that form a \BNG car's body (left panel) and how wheels and suspensions are composed of nodes and beams (right panel).
%
The vehicle models encode the rules that specify how parts are constructed, how they fit together, and how they interact with each other. For example, vehicle models specify how the tires are constructed using nodes and beams and how wheels are attached to the wheel' hubs. Similarly, they describe how the hubs are attached to the suspensions and the chassis' suspensions. The vehicle models also describe how torque propagates from the engine through the car's powertrain (e.g., gearbox, differential, axles) to the wheels.
%
The vehicle models are comprehensive and make \BNG extremely versatile as they allow to model structurally different vehicles in various configurations by directly picking the right parts to assemble them, as it happens in reality. 
%
For instance, according to these models, motorcycles, cars, and trucks need an engine, but trailers do not; motorcycles have two wheels, cars have four, while trucks have more.
%
These models also contain all the necessary logic to simulate headlights, sounds, materials, and the various driving-assistance systems  (e.g., ABS, ESC) that contribute to the final driving simulation and data for realistically render the vehicles.
% ALESSIO: This is a bit confusing since we as talking about physics simulation
% For display purposes, all of the base vehicle physics models are "dressed" with highly detailed 3d graphics meshes that track the motions of the base physics entities.

\textbf{Simulation execution model}.
\BNG implements a two-layered simulation: at high-level, it simulates components that generate forces (e.g., vehicles engines, external controllers) without representing them explicitly as beams and nodes; at low-level, it simulates how the forces propagate across soft-bodies composed of nodes and beams.
%
The simulation execution follows the \textit{actor model}~\cite{10.5555/1624775.1624804}: different vehicles are independent and concurrently executed, and they communicate by passing messages using event queues. Consequently, all the interactions between them happen asynchronously, enabling \BNG to parallelize the physics simulation's execution, the game logic, and the vehicle models on multiple threads, and simulating the force propagation across a large number of elements efficiently.
% 
On top of this layered, ``distributed`` execution model, \BNG can run simulations faster than real-time using gaming setups as well as commodity PCs. 
%
Specifically, on the reference benchmark~\footnote{The reference benchmark is available along with the \BNG's distribution.} 
%\BNG runs the simulations up to five times faster than real-time for one simulated vehicle. We report the results of the reference benchmark in Table~\ref{tab:faster-than-real-time}.

%\begin{table}
%\small
%    \centering
%        \caption{Results of \BNG's reference benchmark in which an increasingly large number of vehicles is concurrently simulated.}
%    \label{tab:faster-than-real-time}
%    \begin{tabular}{r r r} \toprule
%    \multicolumn{1}{c}{\textbf{\# Cars}} & \multicolumn{1}{c}{\textbf{MBeams / sec}} & \multicolumn{1}{c}{\textbf{Real-time speed up}} \\ \midrule
%  nCars  |  | % Realt  |
%     1 &   46.723 &   513\% \\
% 2 &   87.503 &   480\% \\
% 3 &  114.311 &   418\% \\
% 4 &  139.884 &   384\% \\ \bottomrule
%    \end{tabular}
%\footnotesize
%\flushleft{We ran the benchmark using a non-dedicated machine with 16 GB of memory, and an i7 CPU with 4 physical and 4 virtual cores, running at 3.10GHz.} %i7-4770S
%\vspace{-4mm}
%\end{table}

Low-level and high-level simulations are tightly coupled: the components continuously communicate with each other and propagate the forces or torques to the nearby components.
%
Force propagation is bi-directional and happens across both the simulation layers. For example, the low-level physics core calculates the forces acting on a wheel's hub and tire nodes. Next, it passes the angular velocity of the wheel's hub to the high-level drivetrain. Then, the drivetrain propagates the wheel's angular velocity up to the engine that computes the torque. Finally, the engine propagates the torque back to the wheels via the drivetrain, and the physics core applies the torque to the wheel's hub nodes causing the beams that connect it to the tire's nodes to pull them, effectively making the tires move.
%
Similarly, acting on the high-level steering wheel causes a force that propagates through the steering rack and eventually makes the wheels turn. 

%Noticeably, when developers use real steering wheels to drive the simulated vehicles, the simulated wheels' reaction forces are fed back to the steering wheel and realize the so-called force feedback.
%
%Since the simulation continuously propagates forces back and forth across connected components, \BNG ensures the simulation's stability by running the simulation loop at a very high-frequency (up to $2$KHz). 
%This provides a tighter and more stable coupling between the various subsystems. 
%Additionally, because \BNG simulates physics at high-frequency, it can model subtle effects, such as the high-frequency micro-vibrations that happen to the wheels as the tires approach their grip limits, which are notoriously hard to simulate accurately.

% \smallskip
%\begin{figure*}[tp]
%    \centering
%    \includegraphics[width=\textwidth]{crash-example}
%    \caption{ Simulation of the physics, pressure, aerodynamics, and collision of a vehicle in \BNG}
%    \vspace{-2mm}
%    \label{fig:crash-example}
%    \vspace{-3mm}
%\end{figure*}

%\BNG builds on top of the mass-spring approach to soft-body simulation but extends it in many ways to accurately simulate the physics, pressure, aerodynamics, and collisions of entire vehicles (see Figure~\ref{fig:crash-example}). Additionally, the use of comprehensive vehicle models and massively parallel simulation execution enable faster than real-time execution of a large variety of vehicles (see Table~\ref{tab:faster-than-real-time}).

\subsection{Procedural Content Generation with \BNGPY}
\label{sec:beamngpy}
As with many other simulations, \BNG allows users to manually provide additional content to the platform like three-dimensional models, material definitions, and maps.
However, differently than most of the state-of-art simulations, it comes with a set of editors that allow the modification or creation of environmental assets directly inside the platform. It also provides an API that automates scenarios generation, test execution, and data collection and allows external programs to control the simulation. A fundamental requirement for testing driving AIs and implementing test oracles.

\BNGPY organizes simulations around the concept of \emph{scenarios}, driving tasks that the car under tests, (i.e., the \emph{ego-car}) must solve; a common scenario is to drive from a starting location to a target area without driving off-road nor crashing~\cite{intelligence:testing}.
Scenarios take place in \emph{environments} that are defined by a \emph{terrain}, environmental parameters such as \emph{time of day}, and contain \emph{roads} and \emph{static objects} (e.g., props, obstacles).  \BNGPY allows controlling environmental conditions and lighting, the generation of roads, lane markings, curbs, and props' placement and sizing. Like parked cars and traffic signs, complex static objects require the availability of three-dimensional mesh models that define their geometries. Instead, simple objects, like cones and cubes, are procedurally generated.
%

Scenarios involve at least one \emph{ego-car} equipped with sensors, like cameras and \textit{lidars}, and controlled by the driving agent under test. Scenarios might include additional vehicles that can be programmed using \BNGPY. Those non-ego cars implement regular traffic, adversarial scenarios (e.g., cut-in-lane), or critical situations (e.g., car crashes).
%
As for the ego-car, various sensors can be attached to non-ego vehicles to monitor their status. Thanks to those sensors, \BNG fulfills the fundamental ``observability'' requirement of testing, allows the definition of test oracles, and can quickly collect large datasets for training and validation.


==> related-old.tex <==
%\sajad{--here--}


%Autonomous driving is expected to improve transportation safety drastically.
%However, recently reported fatal crashes involving self-driving cars are signaling that, at least in the short-term, these expectations appear to be too optimistic.
%This situation calls for further research in the field to avoid releasing self-driving cars equipped with defective software, which might become erratic and possibly life-threatening.

In this section, we briefly discuss relevant research concerning the following topics: 
\begin{inparaenum}[(i)]
\item academic and industry studies concerning DevOps limitation and practices in the context of general CPSs;
% \item studies concerning testing Deep Neural Networks (DNNs) utilized in SDCs; and
\item studies proposing, using, or evaluating simulation environments for testing SDCs.

\end{inparaenum}
%\sajad{From Alessio: What about related work on fault finding using ML and work on test case selection using ML (and not)}

\subsection{Software Testing Optimization} 
\textbf{Alessio: Add work on Prediction to shorten experiments in CPS Regression Testing and SBST. Example, Lionel's work on using AI and Decisoin Trees, the work of Mullins and Del Guizzo (?) Graz on using Gaussian Processes.
Add the reference to the Survey on test reduction effort}

Research has yielded many approaches to optimize testing. However, most of the available approaches focus on regression testing and found application only in traditional software systems~\cite{Yoo:stvr2010}.  \minor{these approaches can be classified into the following categories: \textit{test case selection}~\cite{Chen:1996}, \textit{test suite reduction, test case minimization)}~\cite{Rothermel:icsm1998}, and \textit{test case prioritization}~\cite{Rothermel:icsm1999}.}

Test case selection approaches identify subsets of available tests relevant (or necessary) for testing a given change in the code.  Test suite reduction approaches remove redundant test cases from existing test suites leading to smaller test suites that can execute faster, while test case minimization approaches remove irrelevant statements from the tests, reducing their size. Finally, test case prioritization approaches rank test cases by the likelihood of detecting faults such that their execution can lead to finding faults soon. 

Compared to traditional software systems, CPSs face additional challenges due to their continuous interactions with the environment and the tight coupling between the hardware and software components comprising them. Consequently, when it comes to testing, standard testing approaches are ineffective, inefficient, or inapplicable~\cite{DBLP:conf/icse/BriandNSB25}.
Testing of CPSs has typically been performed following X-in-the-loop paradigms~\cite{matinnejad2013automated} that in practice takes the form of the \textit{model in the loop} (MiL), \textit{software in the loop} (SiL), and hardware in the loop  (HiL). For MiL testing, most of the software and hardware components, sensors, and other relevant environmental elements are abstracted using models, such that testing can focus on assessing the correctness of the control algorithms governing the CPSs.
For SiL testing, only the hardware components and the environments are abstracted using physically accurate simulators; in this case, the behavior and integration of CPSs software components can be tested in realistic execution conditions. Finally, HiL testing focus on checking the integration of hardware and software components in production-like, either simulated or real, environments. Notably, X-in-the-loop testing involves a great deal of simulation.

Considering the specific need for X-in-the-loop development of CPSs, researchers proposed testing optimization techniques tailored for CPSs \cite{DBLP:journals/tii/ArrietaWMSE18,DBLP:conf/issta/ShinNSBZ18,arrieta2018multi, DBLP:conf/splc/ArrietaWSE16,DBLP:journals/jss/ArrietaWSE19}. 
Test selection (or prioritization) for traditional systems is typically performed by computing the test similarity or test adequacy (i.e., code coverage). However, given the complexity of test inputs for CPSs (e.g., simulated environments), computing traditional similarity metrics based on lexicographic similarity of test code and test inputs is technically challenging and may not be adequate. Consequently, new similarity metrics and procedures to compute them have been proposed recently. For instance, Arrieta \etal~\cite{arrieta2018multi, DBLP:conf/splc/ArrietaWSE16} proposed to measure the similarity between the test cases based on the so-called \textit{signal values} of all the states for the simulation-based test cases. 

Adopting code coverage as a proxy for test adequacy in CPSs systems, which are based on artificial intelligence and deep learning, is not adequate; hence, selecting tests purely driven by code coverage is bound to produce ineffective test suites. Because of this, current research efforts focus on different heuristics to select test cases. Arrieta \etal \cite{DBLP:journals/tii/ArrietaWMSE18} proposed to select test guided by objectives such as requirement coverage and test execution times; they applied test selection in the context of multi-objective test case generation for CPSs and showed improvement over baseline approaches.
Complementary, Shin \etal \cite{DBLP:conf/issta/ShinNSBZ18} proposed an approach for acceptance test selection for a satellite system that selects relevant test cases based on two objectives: (i) the risks of causing hardware damage, and (ii) the number of test cases executed within a given time budget. 

Compared to those studies, we investigate (1) a different CPS domain and (2) different test selection objectives. Specifically, we investigate lane-keeping in self-driving car simulation environments, whereas previous work focused on industrial tanks~\cite{DBLP:journals/jss/ArrietaWSE19, DBLP:journals/tii/ArrietaWMSE18}, satellites~\cite{Shin2018}, electric windows~\cite{arrieta2018multi} and cruise controllers~\cite{DBLP:journals/tii/ArrietaWMSE18}. Regarding test selection objectives, we focus on improving the cost-effectiveness of simulation-based tests to assess safety requirements. In contrast, previous studies prioritized the execution of tests based on their fault-detection capability~\cite{DBLP:journals/jss/ArrietaWSE19}, or selected tests based on signals diversity~\cite{DBLP:journals/tii/ArrietaWMSE18, arrieta2018multi, DBLP:conf/splc/ArrietaWSE16}, that require at least one execution of the test cases in both approaches. Since in the SDC domain, executing simulation-based tests is prohibitive, we face the challenge of selecting test cases before their execution. Consequently, our techniques consider only the initial state of the car and the characteristics of the roads (e.g., geometry, lane markings), as those features are available without executing the tests in the simulator.

% ALESSIO: I comment this out because I do not think this belongs to the Related Work
% The content of the section seems a better fit for the introduction as in contains important elements that motivate this work
% \subsection{Limitations of DevOps for CPSs}

% %from thesis
% % Agile development approach has become the prevalent form.

% %These principles are not limited to traditional software engineering practices and technologies.
% % Their adoption in the context of CPS could benefit the development of CPS \cite{Lwakatare2016}.

% % Currently, the literature for DevOps in CPS is minimal and the CPS pipeline development holds some challenges, specifically in the testing phase.
% % For instance, modeling the hardware in a simulation can be difficult and there are endless possible scenarios and configurations for a CPS that could be tested.
% % Moreover, creating and running such complex test scenarios is not only time consuming, but they also require a lot of resources and are expensive \cite{Arrieta2016AUTO}.


% %from paper
% %The agile development form allows reducing the gap between clients and developers.
% %With the increase of the frequency of software releases, the integration of Development(Dev) and Operations(Ops) functions needed to be tighter. 
% Contemporary
% DevOps pipelines allow improving the communication between Development(Dev) and Operations(Ops) during the software development process, enabling continuous improvements to existing and new products \cite{Hemon2019}.
% Several researchers and practitioners advocate DevOps as a promising approach for CPSs development \cite{antipattern:DevOps,Torngren2018}.
% However, both in traditional \cite{antipattern:DevOps,zampetti:EMSE} and CPS application domains, the state-of-the-art of DevOps is still forming \cite{Torngren2018}, and emerging practices need validation in the wild.\\
% A recent survey by T{\"o}rngren and Sellgren~\cite{Torngren2018} discusses how CPSs' engineering deals with the inner complexity of CPSs' design and the challenges that arise from the environments in which CPSs operate.
% According to them, while (semi-automated) integration happens through software, there are \textbf{\textit{several distinguishing characteristics}} between software and physical systems that make co-designing hardware and software hard.
% Those characteristics include entirely different approaches, techniques, abstractions, platforms, faults \& failure modes, and development practices.
% They conclude that to cope with the foreseen demand of CPSs at scale and in multiple domains, CPS development and testing need rapid prototyping, code/test generation, and various testing phases~\cite{Shokry2009} encapsulating X-in-the Loop (XiL) activities.
% In XiL, the 'X' indicates the target of development and testing and typically refers to model (MiL), software (SiL), and hardware (HiL).
% A typical CPS development pipeline needs to efficiently and effectively integrate various XiL activities to support development and evolution \cite{Torngren2018,Shokry2009}.

% %our contirbution here
% In this paper, we investigated ways to improve XiL activities, by focusing
% on proposing simulation-based test scenario generation and selection approaches for SDCs, equipped with machine-learning-based strategies for enabling the selection of most relevant (or critical) test cases (or scenarios).
% An optimal test case selection needs to target the identification of relevant (i.e., potentially unsafe) test cases, while optimizing simulated testing pipeline, to ensure higher safety for the final products. 

% \subsection{Testing DNNs of Autonomous Systems}
% %from DeepBillboard 
% %needs paraphrasing
% DNNs are being widely applied in many autonomous systems such as SDCs to ensure human-competitive accuracy in cognitive computing tasks. 
% For instance, they are used to map the raw pixels from on-vehicle cameras to the steering control decisions \cite{zhou2020deepbillboard}. 
% Unfortunately, 
% %the reliability and correctness of systems adopting DNNs as part of their control pipeline have not been formally guaranteed. 
% recent DNN testing research has shown that DNNs are rather vulnerable to intentional security attacks, e.g., expressed in form of adversarial inputs with perturbations \cite{carlini2017towards,kurakin2016adversarial}.
% Such adversarial inputs can be digitally crafted by adding malicious perturbations to the original inputs, causing the targeted DNN to output incorrect control decisions \cite{tian2018deeptest,Pei2017,zhang2018deeproad}.
% %There have been multiple research efforts to automate the process for generating adversarial inputs to test SDCs under extreme conditions.

% The literature has produced techniques such as DeepTest \cite{tian2018deeptest}, DeepXplore \cite{Pei2017}, and DeepRoad \cite{zhang2018deeproad} to transform original images to generate adversarial images. The transformation may include different filters or synthesizing different weather or lighting conditions. 
% A further approach, called DeepBillboard \cite{zhou2020deepbillboard},  generates more real test inputs by printing synthetic images on the billboards alongside the road to further test the DNNs under security attacks. Complementary to the above studies, our work does not focus on generating adversarial input images, we focus on generating broad simulated driving scenarios (e.g., including roads, intersections, etc.) using a high accuracy simulation environment, which provides the opportunity to test SDCs in many different settings and simulation dynamics. 

% Stocco {\em et al.} \cite{stocco2019misbehaviour} introduce SelfOracle based on the concept of self-assessment oracle.
% In contrast to the other tools, SelfOracle is used to predict future misbehavior in real-time.
% The oracle monitors the DNN confidence at runtime in order to predict unsupported driving scenarios in advance.
% SelfOracle combines the use of auto-encoder and time-series-based anomaly detection to recreate the previously seen driving scenarios and calculates the confidence boundary of normal or unsupported conditions.\\
% Differently from the work by Stocco {\em et al.}, we do not target \textit{unsupported driving scenarios},  but we rather focus on design and implement strategies able to systematically generate test cases, assessing the behavior of the system in representative  (safe and unsafe) simulation scenarios, while minimizing the costs of the SDCs test simulations.

%\sajad{From Alessio:There are many other works here, not necessarily targeting DNN, Probably also on test selection using ML (Uniqueness of road)}

\subsection{Simulation-based Testing of SDCs}

Given the danger and ineffectiveness of physical testing~\cite{KalraPaddock:2016}, researchers and practitioners devised simulation-based testing approaches for SDCs.
This provides the opportunity to conveniently test the control software of a SDC in a (realistic enough) simulated environment, and in a diverse set of (automatically generated) test cases.  
Additionally, using simulation, the systems under test can face tests that might be otherwise too expensive, too hard, too risky, or impossible to recreate in real life \cite{DosovitskiyRCLK17}.  

Consequently, simulation is becoming one of the cornerstones in developing and validating SDCs, as it is heavily utilized in various XiL activities and across the entire development life-cycle.
Simulation is currently used to support the initial inception and requirement analysis (MiL), Hardware/Software Co-design (MiL), design and testing of software components (SiL), training and validation of Machine Learning components (SiL), and testing and validation of the deployed system (HiL).% add reference for the examples

% \subsubsection{Simulation Environments for Autonomous Systems}

    % \textit{BeamNG} \cite{beamNG} is an open-world vehicle simulator that can be used freely for research purposes.
    % It offers a highly accurate soft-body physics engine, simulating every component of a vehicle in real-time using nodes and beams.
    % This contrasts with most simulators, where often a top-down approach is used, where the physics of the vehicle is specified in its entirety, and the behavior and properties of the components are derived from it.
    % BeamNG also allows users to provide additional content to the platform like three-dimensional models, material definitions, and maps, either manually or via its APIs.
    % These features have made BeamNG the ideal simulation candidate for conducting research aimed at optimizing testing SDCs.
    
    % Testing a CPS requires the generation of test cases that effectively stress the system under tests. To systematically find critical and challenging test cases for the system under test, Gambi {\em et al.} \cite{Gambi2019} combined search-based software testing and procedural content generation into a novel approach called AsFault.
    % AsFault generates road models that stress self-driving cars' lane-keeping and leverages \textbf{BeamNG} to implement them in automatically executed soft-body simulations. 
    % AsFault uses a genetic algorithm to mutate and recombine the road models and create increasingly challenging test scenarios that eventually cause the ego-car to drive off-road.
    
    Abdessalem {\em et al.} \cite{Abdessalem2018} proposed an approach for test scenario generation for SDCs based on a combination of evolutionary search algorithms and decision tree classification models. 
    Their goal is to leverage classification models to guide the search-based generation of tests faster towards critical test cases. 
    Also, search algorithms refine classification models so that the models can accurately characterize critical regions (i.e., the regions of a test input space that are likely to contain the most critical test cases).
    They evaluate their approach by generating test cases for an automated emergency braking system, and use \emph{PreScan} \cite{prescan}, a commercial SDC simulator for the test execution. 
    
    \emph{AV-FUZZER} was proposed by Li {\em et al.} \cite{li2020av}, which consists of a testing framework to find the safety violations of an autonomous vehicle in the presence of an evolving traffic environment.
    They leverage domain knowledge of vehicle dynamics and genetic algorithms to minimize the safety potential of an autonomous vehicle over its projected trajectory and design a local fuzzer that increases the exploitation of local optima in the areas where highly likely safety-hazardous situations are observed.
    For evaluating their proposed framework, They use an Unreal Engine based real-time simulation platform, \emph{LGSVL} \cite{lgsvl}, that is capable of simulating complex urban and freeway driving scenarios using a library of urban layouts, buildings, pedestrians, and vehicles.
    
    Search-based testing struggles to generate test scenarios with peculiar features, e.g., a rear-end car crash, that developers might need to validate or debug their implementations, and manually creating such test scenarios is time-consuming and cumbersome.
    Hence, Gambi {\em et al } devised \textit{AC3R} \cite{Gambi2019Police}, an approach to derive scenario-based tests from simulations of real car crashes.
    AC3R leverages natural language processing and a custom ontology to extract information from police reports that describe car crashes and uses basic kinematics to plan the intercepting vehicles' trajectories. It uses \emph{BeamNG} to automatically simulate the whole environment that re-enacts the car crashes.
    
    % There are several other open-source and commercial simulation environments for self-driving cars that have been used for research on different aspects of SDCs. For instance, \textbf{AirSim} \cite{Shah2017}, \textbf{CARLA} \cite{Dosovitskiy17}, and \textbf{NVidia drive} \cite{nvidia_drive} have been utilized in the literature for simulating drones, cars, and other autonomous systems. 

%our contirbution here
As mentioned before in Section \ref{sec:asfault}, we leveraged AsFault \cite{Gambi2019} to generate test case and BeamnNG \cite{beamNG} to run them in simulation in our study. 
Complementary to such previous studies, we specifically focused on designing and integrating an approach in the SDC testing pipeline, to recognize and exclude safe scenarios \textit{without executing them} based on machine learning models.
This research direction is relevant to save valuable testing and processing resources, and allocate computing power and time to execute more critical (i.e., unsafe) and potentially risky test cases. 
% In future work we are interested to explore the usage of further simulator environments in our simulation pipeline, to increase the impact and generality of our results.



%\subsubsection{Infield testing}
% Self-driving cars receive data from different sensors and use a Deep Neural Network (DNN) to determine the driving parameters and expected behaviours.
% Companies are conducting infields tests with real cars in test facilities or real-world roads to test such complex systems \cite{Cerf2018}.
% During the infield tests, they are collecting detailed sensor data, which can be recorded and played back.
% The recorded data can further be used in simulations to create comprehensive situational testing\cite{Cerf2018}.
% A major challenge in testing self-driving cars is the unlimited number of testable scenarios combined with the internal functioning of DNNs, which are lack interpretability for humans \cite{stocco2019misbehaviour}.
% There have been different approaches to tackle this challenge using synthesized inputs and simulations.

%\subsection{Test Case Selection in Complex Systems}
%\seba{Here we need to add references to it..}
